Bound-electron self-energy calculations in Feynman and Coulomb gauges: detailed analysis

The energy correction associated with the self-energy diagram is the leading (in magnitude) and fundamental (in significance) contribution to the Lamb shift in highly charged ions. Conventional approaches to this correction rely on partial-wave expansions, which is a stumbling block limiting accuracy. To elucidate the issue, we perform a comprehensive comparative analysis of partial-wave-expansion convergence between two gauges: Feynman and Coulomb. Some tricks for improving the convergence are discussed as well.

==> contribs_mp_tricks.tex <==
{\setlength\LTcapwidth{\textwidth}
\renewcommand{\arraystretch}{1.8}
\setlength{\tabcolsep}{1pt}
\begin{table}[h]
    \centering
    \caption{\label{tab:contribs_mp_tricks}
        Many-potential term and the self-energy correction for the ground state of hydrogen-like argon. Comparison of two acceleration tricks and two gauges, Feynman (F) and Coulomb (C) (in eV).
        The individual terms of the partial-wave expansion for the many-potential contribution as well as
        the results of applying the extrapolation procedure are shown. The nuclear-charge distribution is described by the homogeneously-charged-sphere model with the root-mean-square radii taken from \cite{hen}.
         }
% \resizebox{\textwidth}{!}{
{
{\fontsize{8pt}{8pt}\selectfont{
    \begin{tabular}{
                l@{\quad}
                S[table-format=-3.8(2),group-separator={},group-minimum-digits=3]
                S[table-format=-3.8(2),group-separator={},group-minimum-digits=3]
                S[table-format=-3.8(2),group-separator={},group-minimum-digits=3]
                S[table-format=-3.8(2),group-separator={},group-minimum-digits=3]
                S[table-format=-3.8(2),group-separator={},group-minimum-digits=3]
                S[table-format=-3.8(2),group-separator={},group-minimum-digits=3]
                }
\hline
\hline
& \multicolumn{3}{c}{F} & \multicolumn{3}{c}{C} \\ 
% \hline 
% \hline
% $\Delta \varepsilon_a^{0p}+\Delta \varepsilon_a^{1p}$ & &  -18.413 394 4 & & & 1.396 437 4 & \\
\hline
& \multicolumn{1}{c}{$\Delta {\varepsilon}_a^{\text{Mp}}$} & \multicolumn{1}{c}{$\Delta {\varepsilon}_a^{3+}$} & \multicolumn{1}{c}{$\Delta \tilde{\varepsilon}_a^{3+}$} & \multicolumn{1}{c}{$\Delta {\varepsilon}_a^{\text{Mp}}$} & \multicolumn{1}{c}{$\Delta {\varepsilon}_a^{3+}$} & \multicolumn{1}{c}{$\Delta \tilde{\varepsilon}_a^{3+}$}\\
\hline
substr. &  & 8.960 544 04(15) & 8.722 252 3 &  & -0.155 550 67(9) & -0.218 341 8\\
\hline
$|\kappa| = 1$ 
  &    18.954139  &        10.6306576      &     10.8509659   &    -0.098735 &    -0.01593568 &     0.0408756   \\
$2$ &   0.447224  &         0.0333412      &      0.0491332   &    -0.044326 &    -0.00662752 &    -0.0016441   \\
$3$ &   0.115257  &         0.0042399      &      0.0059313   &    -0.011632 &    -0.00061625 &     0.0000173   \\
$4$ &   0.046658  &         0.0010336      &      0.0013902   &    -0.006453 &    -0.00026991 &    -0.0000776   \\
$5$ &   0.023375  &         0.0003404      &      0.0004394   &    -0.004153 &    -0.00015126 &    -0.0000734   \\
$6$ &   0.013267  &         0.0001294      &      0.0001612   &    -0.002872 &    -0.00009440 &    -0.0000571   \\
$7$ &   0.008186  &         0.0000519      &      0.0000628   &    -0.002080 &    -0.00006308 &    -0.0000431   \\
$8$ &   0.005368  &         0.0000201      &      0.0000238   &    -0.001558 &    -0.00004428 &    -0.0000326   \\
$9$ &   0.003688  &         0.0000062      &      0.0000017   &    -0.001199 &    -0.00003229 &    -0.0000250   \\
$10$ &  0.002630  &        -0.0000000      &      0.0000000   &    -0.000943 &    -0.00002426 &    -0.0000195   \\
$11$ &  0.001933  &        -0.0000028      &     -0.0000030   &    -0.000754 &    -0.00001868 &    -0.0000155   \\
$12$ &  0.001458  &        -0.0000039      &     -0.0000042   &    -0.000613 &    -0.00001469 &    -0.0000124   \\
$13$ &  0.001124  &        -0.0000042      &     -0.0000046   &    -0.000505 &    -0.00001175 &    -0.0000101   \\
$14$ &  0.000882  &        -0.0000042      &     -0.0000044   &    -0.000420 &    -0.00000955 &    -0.0000084   \\
$15$ &  0.000704  &        -0.0000039      &     -0.0000042   &    -0.000353 &    -0.00000786 &    -0.0000070   \\
$16$ &  0.000570  &        -0.0000036      &     -0.0000038   &    -0.000300 &    -0.00000655 &    -0.0000058   \\
$17$ &  0.000468  &        -0.0000033      &     -0.0000034   &    -0.000257 &    -0.00000551 &    -0.0000050   \\
$18$ &  0.000388  &        -0.0000030      &     -0.0000031   &    -0.000221 &    -0.00000468 &    -0.0000042   \\
$19$ &  0.000325  &        -0.0000027      &     -0.0000028   &    -0.000192 &    -0.00000400 &    -0.0000036   \\
$20$ &  0.000275  &        -0.0000024      &     -0.0000025   &    -0.000168 &    -0.00000345 &    -0.0000032   \\
$21$ &  0.000234  &        -0.0000021      &     -0.0000022   &    -0.000147 &    -0.00000300 &    -0.0000028   \\
$22$ &  0.000201  &        -0.0000019      &     -0.0000020   &    -0.000130 &    -0.00000262 &    -0.0000024   \\
$23$ &  0.000174  &        -0.0000017      &     -0.0000018   &    -0.000115 &    -0.00000230 &    -0.0000021   \\
$24$ &  0.000152  &        -0.0000016      &     -0.0000016   &    -0.000103 &    -0.00000203 &    -0.0000019   \\
$\sum_{k=1}^{24}$ & 19.628 680 & 10.669 779 0 & 10.908 065 9 & -0.178 229 & -0.023 955 60 & 0.038 836 1  \\
$\sum_{k=25}^{\infty}$ [extr.] & 0.001 61(1) & -0.000 022 5(6) & -0.0000171(4) & -0.00130(1) & -0.00002438(12) & -0.0000247(2) \\
% $\Delta \varepsilon_a^{temp}$ & 19.630 29(1) & 10.669 756 5(6) & 10.908 048 8(4) & -0.179 53(1) & -0.023 979 98(12) & 0.038 811 4(2) \\
\hline
$\Delta \varepsilon_a^{\text{Mp}}$ &     19.63029(1)         &    19.630 300 6(7)          &    19.630 301 2(4)        &     -0.179 53(1)         &   -0.179 530 8(2)   &   -0.179 530 6(2)    \\
\hline
$\Delta \varepsilon_a$ & 1.216 89(1) & 1.216 906 2(7) & 1.216 906 8(4) & 1.216 91(1)  & 1.216 906 6(2) & 1.216 906 8(2)\\
\hline 
\cite{hen} & 1.216 90(1) & 1.216 90(1) & 1.216 90(1) & 1.216 901(3)  & 1.216 901(3) & 1.216 901(3)\\
\hline 
\hline
\end{tabular}
}}}
\end{table}
}









==> results_v1.tex <==
\textcolor{red}{///////////////////////////////// START OF V1 // WHAT WAS BEFORE ////////////////////}

\textcolor{red}{Corresponding figs: ~\ref{fig:mp_contributions}, ~\ref{fig:decreasing_powers}
}


We denote by $\Delta \varepsilon_a^{\text{Mp}}(k)$ the contribution to $\Delta \varepsilon_a^{\text{Mp}}$ corresponding to the given $k$ (thus, the partial sum $S_k$ is $S_k = \sum_{k'=1}^k\Delta \varepsilon_a^{\text{Mp}}(k')$). In Fig.~\ref{fig:mp_contributions} the individual $k$ terms of the PW expansion of the many-potential contribution from Tab.~\ref{tab:contribs_mp} are plotted on a log-log scale, for negative values the absolute value is shown. Fig.~\ref{fig:mp_contributions}(a) demonstrates the pros and cons of using the Coulomb gauge versus the Feynman one. For low nuclear charges (see $Z=18$), the magnitude of the individual terms obtained in the Feynman gauge is significantly larger than that of those obtained in the Coulomb gauge. However, this is compensated by the rate of decay of the values. For instance, at $k=20$ the contributions are of the same order of magnitude. For high nuclear charges (see $Z=92$), we have almost the same rate of decay. Nevertheless, the individual contributions $\Delta \varepsilon_a^{\text{Mp}}(k)$ in the Feynman gauge are still larger in absolute value.

=====

\begin{figure}[h!]
    \begin{minipage}[h]{0.49\textwidth}
        \center{\includegraphics[width=0.99\textwidth]{graphs_new/z18_92_2+_normalized(fullSE)_mine.jpg} \\ (a)}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.49\textwidth}
\center{\includegraphics[width=0.99\textwidth]{graphs_new/z18_92_2+_normalized(kp=10)_mine.jpg} \\ (b)}
    \end{minipage}
    \caption{Comparison of contributions of $k$ expansion of many-potential term. Note the log-log scale.}
     % (a): normalized to the total self-energy correction, (b): normalized to $\Delta \varepsilon_a^{mp}(k=10)$. 
\label{fig:mp_contributions}
\end{figure}

Normalizing to a specific contribution, such as $\Delta \varepsilon_a^{\text{Mp}}(10)$ in Fig.~\ref{fig:mp_contributions}b, allows a much closer comparison of the decay rates of contributions. In the log-log scale, the slope of the graph corresponds to the leading power $p$ in the asymptotics $\Delta \varepsilon_a^{\text{Mp}}(k) \sim \frac{1}{\kappa^p}$. We thus consider the power of $p$ as a function of $k$, that could be calculated using the approximate expression:

\begin{equation}
    p(k) = -\frac{k  df}{f dk} \approx -\frac{\ln f(k + 1) - \ln f(k)}{\ln (k + 1) - \ln k},
    \label{eq:p_power}
\end{equation}
where $f = f(k) = \Delta \varepsilon_a^{mp}(k)$.
The function $p(k)$ allows one to extract the leading asymptotics of the contributions; its estimation for hydrogen-like argon, xenon, and uranium in both gauges is presented in Fig.~\ref{fig:decreasing_powers}. As follows from that graph, we have a convergence of $p(\kappa)$ to $3$ in all cases. Thus, the smallest power, used in $k$ extrapolation in~(\ref{eq:kappa_expansion}), should be $\frac{1}{k^2}$ (since $\sum_{k=1}^{n} \frac{1}{k^3} \sim \frac{1}{n^2}$). In the large-$Z$ region $p$ depends weakly on gauge, however in the low-$Z$ region, in the Coulomb gauge $p(k)$ takes on much smaller values than in the Feynman gauge. But the contributions $\Delta \varepsilon_a^{\text{Mp}}(k)$ in the Coulomb gauge have smaller absolute values too. The latter circumstance balances the slow convergence and makes the Coulomb and Feynman gauges equally suitable for estimating the many-potential term in the SE correction for all $Z$.

% The last circumstance overcomes the slow convergence and makes the Coulomb gauge slightly better for estimating the SE correction.

\begin{figure}[H]
    \centering
\includegraphics[width=0.6\linewidth]{graphs_new/ins_degree.png}
    \caption{Power $p$ of decay of contributions to the many-potential contribution as a function of $k$}
    \label{fig:decreasing_powers}
\end{figure} 


\textcolor{red}{////////////////////////////////////////////////////////////////////////}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% START OF V1 // WHAT WAS BEFORE %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Notes on the acceleration-convergence schemes}

\textcolor{red}{///////////////////////////////// START OF V1 // WHAT WAS BEFORE ////////////////////}

\textcolor{red}{
Corresponding figs: ~\ref{fig:mp_contributions1}
}

Now let us turn to the comparative analysis of the SC and two-potential schemes. First, in Fig.~\ref{fig:mp_contributions1}a the ratio of the (quasi-) three-plus-potential contributions (denoted as $S_\infty^{(3+)}$) to the many-potential contribution ($S_\infty^{\text{Mp}}$) is plotted. 
% We call this the deviation of the coefficient $S_\infty$ (taken from the the Eq.~(\ref{eq:kappa_expansion})). 

\begin{figure}[h!]
    \begin{minipage}[h]{0.49\textwidth}
        \center{\includegraphics[width=0.99\textwidth]{graphs_new/C0_deviation.jpg} \\ (a)}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.49\textwidth}
        \center{\includegraphics[width=0.99\textwidth]{graphs_new/C2_deviation.jpg} \\ (b)}
    \end{minipage}
    \caption{Deviations of extrapolation coefficients $S_\infty$, $C_2$ for (quasi-) three-plus-potential terms, $S_\infty$ (a) is the extrapolated sum of the series, and $C_2$ (b) is the leading power ($\sim \frac{1}{k^2}$) coefficient. \textcolor{red}{тут кстати z10 убрать слева}}
    \label{fig:mp_contributions1}
\end{figure}

It is evident that in the small-$Z$ region the two-potential scheme yields the smallest three-plus-potential contribution to be extrapolated. However, the accuracy there is limited by the remainder -- the two-potential contribution itself. Therefore, for small $Z$ the combination of the Coulomb gauge and the Sapistein-Cheng scheme works better. The non-monotonicity of the blue graph is explained by the fact that the quasi-three-plus potential contribution passes through zero and changes sign. 

Let us discuss the extrapolation coefficients $C_i$ from Eq.~(\ref{eq:kappa_expansion}). From our study it follows that the error in the extrapolation coefficients grows quite rapidly with increasing $i$. 
Therefore, we consider the deviation of the first expansion coefficient $C_2$, plotted in~\ref{fig:mp_contributions1}b. This coefficient is also the most significant in the asymptotics of large $k$. Subtraction of (quasi-) two-potential contributions does indeed allow us to reduce the value of the coefficient $C_2$, especially in the region of small $Z$ (by one or two orders of magnitude), which improves convergence. In the large-$Z$ region, the acceleration schemes in the Coulomb gauge work much better and allow one to obtain the many-potential contribution more accurately (see Tab.~\ref{tab:we_yerokh_2p}). It can be seen that both schemes produce almost identical values of $C_2$ (within the same gauge), their difference \textcolor{green}{(from Egor) with the coefficient obtained from the whole many-potential term $\Delta \varepsilon_a^{\text{Mp}}$} is usually greater than the error in their determination. We cannot conclude that the extraction of two-potential contributions reduces the minimum power in the expansion~(\ref{eq:kappa_expansion}) to 3; we argue that the opposite situation occurs. The last statement has been verified empirically -- the extrapolation procedure gave incorrect results. An example of the application of the acceleration-convergence scheme for argon ($Z=18$) is given in Tab.~\ref{tab:contribs_mp_tricks}. 


(However, this is compensated by the rate of decay of the values. For instance, at $k=20$ the contributions are of the same order of magnitude)

(это не про rate, они просто выравниваются; only X times larger)

==> results_v2.tex <==
\textcolor{red}{////////////////////////// START OF V2 // WHAT I SUGGEST ///////////////////////}
\textcolor{red}{
Corresponding figs: ~\ref{fig:mp_contributions_new}
}


We denote by $\Delta \varepsilon_a^{\text{Mp}}(k)$ the contribution to $\Delta \varepsilon_a^{\text{Mp}}$ corresponding to the given $k$ (thus, the partial sum $S_k$ is $S_k = \sum_{k'=1}^k\Delta \varepsilon_a^{\text{Mp}}(k')$). In Fig.~\ref{fig:mp_contributions_new} the individual $k$ terms of the PW expansion of the many-potential contribution from Tab.~\ref{tab:contribs_mp} normalized to the full self-energy correction $\Delta \varepsilon_a$ are plotted on a log-log scale, for negative values the absolute value is shown. This kind of normalization let us see what portion of full self-energy correction is obtained by each contribution. The slope of the graph corresponds to the leading power in the asymptotics. Fig.~\ref{fig:mp_contributions_new}(b) demonstrates  these asymptotics by plotting $\Delta \varepsilon_a^{\text{Mp}}(k)\cdot k^3$. Every data series approaches to a constant which determines the leading asymptotic of the contributions $\Delta\varepsilon_a^{\text{Mp}}(k)\sim\frac{1}{k^3}$ regardless of gauge and nuclear charge $Z$. This result justifies the form of extrapolation ansatz we use for partial sums~\eqref{eq:kappa_expansion}.

For low nuclear charges (see $Z=18$), the magnitude of the individual terms obtained in the Feynman gauge is significantly larger than that of those obtained in the Coulomb gauge. However, this is compensated by the rate of decay of the values: in the Coulomb gauge contributions reach their asymptotic behavior more slowly. For instance, at $k=20$ the contributions in both gauges are of the same order of magnitude. For high nuclear charges (see $Z=92$), we have almost the same rate of decay. Nevertheless, the individual contributions $\Delta \varepsilon_a^{\text{Mp}}(k)$ in the Feynman gauge are still larger in absolute value. These circumstances balances slightly different decay rates and magnitudes, therefore, the Coulomb and Feynman gauges are equally suitable for estimating the many-potential term in the SE correction for all $Z$.

% Normalizing to the full self-energy correction $\Delta \varepsilon_a$ in Fig.~\ref{fig:mp_contributions_new} allows for a much closer comparison of the decay rates of contributions. On the log-log scale, the slope of the graph corresponds to the leading power in the asymptotics. Fig.~\ref{fig:mp_contributions_new}(b) demonstrates  these asymptotics by plotting $\Delta \varepsilon_a^{\text{Mp}}(k)\cdot k^3$. Every data series approaches to a constant which determines the leading asymptotic of the contributions $\Delta\varepsilon_a^{\text{Mp}}(k)\sim\frac{1}{k^3}$ regardless of gauge and nuclear charge $Z$. However, one can note that contributions in the Coulomb gauge have smaller absolute values. Another important feature is that contributions in the Coulomb gauge reach their asymptotic behavior more slowly especially for lower values of nuclear charge $Z$. 

\begin{figure}[h!]
    \begin{minipage}[h]{0.49\textwidth}
        \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_2+_normalized(full_se).jpg} \\ (a)}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.49\textwidth}
\center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_2+_normalized(full_se)_kp3.jpg} \\ (b)}
    \end{minipage}
    \caption{Comparison of contributions of $k$ expansion of 2+ many-potential term in the log-log scale. (a): exact values of contributions, (b): contributions multiplied by $k^3$ to show the main asymptotic.}
     % (a): normalized to the total self-energy correction, (b): normalized to $\Delta \varepsilon_a^{mp}(k=10)$. 
\label{fig:mp_contributions_new}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% START OF V2 // WHAT I SUGGEST %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Notes on the acceleration-convergence schemes V2}

\textcolor{red}{////////////////////////// START OF V2 // WHAT I SUGGEST ///////////////////////}

\textcolor{red}{
Corresponding figs: ~\ref{fig:q3+_contributions},~\ref{fig:mp_contributions2}
}

\textcolor{green}{These two figures show that both schemes gives almost the same contributions of 3+ potential term. And they are also good to compare with the similar picture for 2+ many-potential. I'm thinking how to implement this idea into the article.}

% Now let us turn to the comparative analysis of the SC and two-potential schemes. First, in Fig.~\ref{fig:3+_contributions} the contributions of the accelerated 3+potential series are plotted. Comparing this with Fig.~\ref{fig:mp_contributions1}, one perceives that the contributions of the series accelerated by both schemes and the non-accelerated series have the same leading power of $\frac{1}{k^3}$. By using acceleration schemes, we obtain lower magnitudes of contributions only by a constant factor less than unity, but their decay has the same asymptotic behavior.

Now let us turn to the comparative analysis of the SC and two-potential schemes. On the Fig.~\ref{fig:q3+_contributions} there are plotted individual terms for $Z=18$ of both accelerated series: first is obtained with using Sapirstein-Cheng scheme (a, b), second is obtained with two-potential scheme (c, d). There is uses the same normalization as before in Fig.~\ref{fig:mp_contributions_new}.
 % Direct values of these terms are given explicitly in Tab.~\ref{tab:contribs_mp_tricks}.
There are also shown the absolute values of contributions, therefore, peaks with extremely low values are the point where contributions of accelerated series change their sign. (b, d) demonstrates the same asymptotic behavior $\propto \dfrac{1}{k^3}$ of contributions which we have already seen in Fig.~\ref{fig:mp_contributions_new}. Note, that the main difference between two schemes lies into the low $k$ region, up to $k \approx 5$. This leads to different values for the sums of the series presented as $S_\infty$ but similar other coefficients of extrapolation we obtained. 

The detailed analysis of partial sum extrapolation is presented in Fig.~\ref{fig:mp_contributions2}. There are given the values of how different extrapolation coefficients for accelerated series are from coefficients of extrapolation of non-accelerated series. There are two main points similar for both schemes in both gauges. First, the sum of accelerated series is less in magnitude than the sum of non-accelerated one which comes from $\bigg| \dfrac{S_\infty^{3+}}{S_\infty^{2+}} \bigg| < 1$ for all $Z$. The second thing is that the $C^{3+}_2$ is not vanish in accelerated series. This coefficient is close to $0$ in the low $Z$ region. However, its high uncertainty disallow us to put it equal to $0$. The main difference in results for these schemes is the values of $S_\infty$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Full abcd picture
% \begin{figure}[h!]
%     \begin{minipage}[h]{0.49\textwidth}
%         \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_q3+_normalized(full_se).jpg} \\ (a)}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[h]{0.49\textwidth}
%         \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_q3+_normalized(full_se)_kp3.jpg} \\ (b)}
%     \end{minipage}
%     \\
%     \begin{minipage}[h]{0.49\textwidth}
%         \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_3+_normalized(full_se).jpg} \\ (c)}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[h]{0.49\textwidth}
%         \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_3+_normalized(full_se)_kp3.jpg} \\ (d)}
%     \end{minipage}
%     \caption{Comparison of contributions of $k$ expansion of quasi-3+ many-potential term obtained by Sapirstein-Cheng scheme in the log-log scale. (a): exact values of contributions, (b): contributions multiplied by $k^3$ to show the main asymptotic. (c) and (d) are built for 2-potential scheme: exact values and with multiplication.}
%     \label{fig:3+_contributions}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h!] 
        \center{\includegraphics[width=0.4\textwidth]{graphs_test/z18_3+_normalized.png}}
    \caption{Comparison of individual terms of $k$ expansion of quasi-3+ many-potential term obtained by Sapirstein-Cheng (SC) and Artemyev (TP) schemes in the log-log scale. These contributions are multiplied by $k^3$ to extract main asymptotic.}
    \label{fig:3+_contributions}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{figure}[h!]
%     \begin{minipage}[h]{0.49\textwidth}
%         \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_3+_normalized(full_se).jpg} \\ (a)}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[h]{0.49\textwidth}
%         \center{\includegraphics[width=0.99\textwidth]{graphs_test/z18_92_3+_normalized(full_se)_kp3.jpg} \\ (b)}
%     \end{minipage}
%     \caption{Comparison of contributions of $k$ expansion of 3+ many-potential term obtained by 2-potential scheme in the log-log scale. (a): exact values of contributions, (b): contributions multiplied by $k^3$ to show the main asymptotic.}
%     \label{fig:3+_contributions}
% \end{figure}

\begin{figure}[h!]
    \begin{minipage}[h]{0.49\textwidth}
        \center{\includegraphics[width=0.99\textwidth]{graphs_test/s_inf_no_errors.png} \\ (a)}
    \end{minipage}
    \hfill
    \begin{minipage}[h]{0.49\textwidth}
        \center{\includegraphics[width=0.99\textwidth]{graphs_test/C_2_no_errors.png} \\ (b)}
    \end{minipage}
    \caption{Parts of extrapolation coefficients $S_\infty$ and $C_2$ for (quasi-) three-plus-potential terms in the whole two-plus-potential term: (a) the extrapolated sum $S_\infty$ of the series and (b) the coefficient $C_2$ before the leading power $\dfrac{1}{k^2}$.}
    \label{fig:mp_contributions2}
\end{figure}

\textcolor{red}{////////////////////////////////////////////////////////////////////////}


==> we_sw_2p.tex <==
{\setlength\LTcapwidth{\textwidth}
\renewcommand{\arraystretch}{1.93}
\setlength{\tabcolsep}{1pt}
\begin{table}[h]
    \centering
    \caption{\label{tab:we_sw_2p}
         Many-potential contribution to the self-energy correction for the $1S_{1/2}$  state of hydrogen-like ions (in eV), calculated in three ways: directly, (using the separation of the two-potential contribution), and (using the Sapirstein-Cheng (SC) approach). 
         The nuclear-charge distribution is described by the homogeneously-charged-sphere model with the root-mean-square radii taken from~\cite{hen}.
         }
\resizebox{\textwidth}{!}{
{\fontsize{12pt}{12pt}\selectfont{
    \begin{tabular}{
                l@{\quad}
                l@{\quad}
                l@{\quad}
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                }
    \hline
    \hline 
    
    & & & \multicolumn{1}{c}{direct} & \multicolumn{3}{c}{two-pot. scheme} & \multicolumn{3}{c}{SC scheme} \\
     
    \hline
    
    \multicolumn{1}{l}{$Z$} & 
    \multicolumn{1}{l}{gauge} & &
    \multicolumn{1}{c}{$\Delta\varepsilon^{\text{Mp}}_a$} &
    \multicolumn{1}{c}{$\Delta\varepsilon^{2\text{p}}_a$} & 
    \multicolumn{1}{c}{$\Delta\varepsilon^{3+}_a$} &
    \multicolumn{1}{c}{$\Delta\varepsilon^{\text{Mp}}_a$} &
    \multicolumn{1}{c}{$\Delta \tilde{\varepsilon}_{a,p}^{2\text{p}}$} &
    \multicolumn{1}{c}{$\Delta \tilde{\varepsilon}_{a}^{3+}$} &
    \multicolumn{1}{c}{$\Delta \varepsilon_a^{\text{Mp}}$} \\

    \hline 
    
    18 & C & DKB & -0.179 4(1) &  &  &  & {\multirow{2}{*}{\tablenum{-0.218 341 8}}} & 0.038 82(2) & -0.179 52(2) \\
      &  & GF & -0.179 53(1)  & -0.155 550 67(9) & -0.023 979 98(12) & -0.179 530 8(2) & & 0.038 811 4(2) & -0.179 530 6(2) \\
      & F & DKB & 19.630(1) &  &  &  & {\multirow{2}{*}{\tablenum{8.722 252 3}}} & 10.908 0(1) & 19.630 2(1) \\ 
      &  & GF & 19.630 29(1) & 8.960 544 04(15) & 10.669 756 5(6) & 19.630 300 6(7) & & 10.908 048 8(4) & 19.630 301 2(4) \\ \hline
     54 & C & DKB & -9.982(1) &  &  & & {\multirow{2}{*}{\tablenum{-7.403 692}}} & -2.577 7(2) & -9.981 3(2) \\
      &  & GF & -9.981 32(2) & -6.727 056 62(3) & -3.254 253(2) & -9.981 31(2) & & -2.577 618(3) & -9.981 311(3) \\
      & F & DKB & 145.731(2) &  &  &  & {\multirow{2}{*}{\tablenum{54.420 120}}} & 91.313 7(7) & 145.733 8(7) \\ 
      &  & GF & 145.733 84(4) & 55.334 247 46(3) & 90.399 623(7) & 145.733 871(7) & & 91.313 751(3) & 145.733 872(3) \\ \hline
     92 & C & DKB & -68.764(3) &  &  & & {\multirow{2}{*}{\tablenum{-23.349 279}}} & -45.415 6(8) & -68.764 8(8) \\
      &  & GF & -68.764 1(2)  & -31.829 260 86(19) & -36.934 883(6) & -68.764 144(6) & &  -45.414 865(5) & -68.764 144(5) \\
      & F & DKB & 399.36(1) &  &  & & {\multirow{2}{*}{\tablenum{149.189 230}}} & 250.175(7) & 399.364(7) \\ 
      &  & GF & 399.361 141(11) & 144.424 324 42(12) & 254.936 814(17) & 399.361 138(17) & &  250.171 912(15) & 399.361 142(15) \\
    
  \hline 
  \hline
 
\end{tabular}
}}}
\end{table}
}


==> we_sw_general.tex <==
{\setlength\LTcapwidth{\textwidth}
\renewcommand{\arraystretch}{1.40}
\begin{table}[h]
    \centering
    \caption{\label{tab:we_sw_general}
         Individual contributions to the self-energy correction for the $1S_{1/2}$  state of hydrogen-like ions in the Feynman (F) and Coulomb (C) gauges (in eV). 
         The nuclear-charge distribution is described by the homogeneously-charged-sphere model with the root-mean-square radii taken from \cite{hen}.
         }
{
    \begin{tabular}{
                l@{\quad}
                l@{\quad}
                l@{\quad}
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                 }
\hline
\hline 

\multicolumn{1}{l}{$Z$} & 
\multicolumn{1}{l}{gauge} & &
\multicolumn{1}{c}{$\Delta \varepsilon_a^{0\text{p}}$} &
\multicolumn{1}{c}{$\Delta \varepsilon_a^{1\text{p}}$} & 
\multicolumn{1}{c}{$\Delta \varepsilon_a^{\text{Mp}}$} &
\multicolumn{1}{c}{$\Delta \varepsilon_a$} \\
\hline 
18 & C & DKB     & {\multirow{2}{*}{\tablenum{1.341 667 2}}} & {\multirow{2}{*}{\tablenum{0.054 770 2}}} & -0.179 52(2) & 1.216 91(2) \\ 
&  & GF         & & & -0.179 530 8(2) & 1.216 906 6(2) \\ 
&  & {\cite{hen}} & 1.341 668 068(1) & 0.054 770 997(7) & -0.179 538(3) & 1.216 901(3) \\ 
\hline 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-67.924 836 7}}} & {\multirow{2}{*}{\tablenum{49.511 442 3}}} & 19.630 2(1) & 1.216 8(1) \\ 
 &  & GF         & & & 19.630 301 2(4) & 1.216 906 8(4) \\ 
 &  & \cite{hen} & -67.924 837 74(5) & 49.511 443 05(6) & 19.630 296(10) & 1.216 90(1) \\ 
\hline 
54 & C & DKB     & {\multirow{2}{*}{\tablenum{43.590 610}}} & {\multirow{2}{*}{\tablenum{17.387 958}}} & -9.981 3(2) & 50.997 2(2) \\ 
 &  & GF         & & & -9.981 311(3) & 50.997 257(2) \\ 
 &  & \cite{hen} & 43.590 621 48(6) & 17.387 986 7(3) & -9.981 343(16) & 50.997 27(2) \\ 
\hline 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-285.092 638}}} & {\multirow{2}{*}{\tablenum{190.356 023}}} & 145.733 8(7) & 50.997 1(7) \\ 
 &  & GF         & & & 145.733 872(3) & 50.997 257(3) \\ 
 &  & \cite{hen} & -285.092 638 6(1) & 190.356 052 0(3) & 145.733 90(8) & 50.997 31(8) \\ 
\hline 
92 & C & DKB     & {\multirow{2}{*}{\tablenum{210.068 167}}} & {\multirow{2}{*}{\tablenum{213.738 955}}} & -68.764 8(8) & 355.042 3(8) \\ 
 &  & GF         & & & -68.764 144(5) & 355.042 978(5) \\ 
 &  & \cite{hen} & 210.068 220 5(7) & 213.739 094(4) & -68.764 3(1) & 355.043 0(1) \\ 
\hline 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-516.318 629}}} & {\multirow{2}{*}{\tablenum{472.000 467}}} & 399.364(7) & 355.045(7) \\ 
 &  & GF         & & & 399.361 141(11) & 355.042 979(11) \\ 
 &  & \cite{hen} & -516.318 598(4) & 472.000 597(6) & 399.361 2(2) & 355.043 2(2) \\ 
 \hline 
 \hline 

\end{tabular}
}
\end{table}
}

==> we_yerokh_2p.tex <==
{\setlength\LTcapwidth{\textwidth}
\renewcommand{\arraystretch}{2.1}
\setlength{\tabcolsep}{1pt}
\begin{table}[h]
    \centering
    \caption{\label{tab:we_yerokh_2p}
         Many-potential contribution to the self-energy correction for the $1S_{1/2}$  state of hydrogen-like ions, calculated in three ways: directly, (using the separation of the two-potential contribution), and (using the Sapirstein-Cheng (SC) approach). Results are given in units $F(\alpha Z)$. For $Z=10$ spherical model was used, and for other $Z$'s Fermi model was used, nuclear radii taken from~\cite{se_yerokh}.
         }
\resizebox{\textwidth}{!}{
{\fontsize{12pt}{12pt}\selectfont{
    \begin{tabular}{
                l@{\quad}
                l@{\quad}
                l@{\quad}
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.10(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                }
    \hline
    \hline 
    
    & & & \multicolumn{1}{|c|}{direct} & \multicolumn{3}{c}{two-pot. scheme} & \multicolumn{3}{|c}{SC scheme} \\
     
    \hline
    
    \multicolumn{1}{l}{$Z$} & 
    \multicolumn{1}{l}{gauge} & &
    \multicolumn{1}{c}{$\Delta\varepsilon^{\text{Mp}}_a$} &
    \multicolumn{1}{c}{$\Delta\varepsilon^{2\text{p}}_a$} & 
    \multicolumn{1}{c}{$\Delta\varepsilon^{3+}_a$} &
    \multicolumn{1}{c}{$\Delta\varepsilon^{\text{Mp}}_a$} &
    \multicolumn{1}{c}{$\Delta \tilde{\varepsilon}_{a,p}^{2\text{p}}$} &
    \multicolumn{1}{c}{$\Delta \tilde{\varepsilon}_{a}^{3+}$} &
    \multicolumn{1}{c}{$\Delta \varepsilon_a^{\text{Mp}}$} \\
    \hline 
    10 & C & DKB & -0.570 0(8) &  &  &  & {\multirow{2}{*}{\tablenum{-0.791 761 7}}}& 0.221 95(5) & -0.569 81(5) \\
  &  & GF & -0.569 8(1)  & -0.519 43(2) & -0.050 350 0(1) & -0.569 78(2) & & 0.221 992 9(1) & -0.569 768 8(1) \\
  & F & DKB & 188.7(6) &  &  &  & {\multirow{2}{*}{\tablenum{87.239 75}}}& 101.435 75(2) & 188.675 50(2) \\ 
  &  & GF & 188.675 3(2) & 89.835 999(2) & 98.839 47(1) & 188.675 47(1) & & 101.435 74(2) & 188.675 49(2) \\ 
\hline
 18 & C & DKB & -0.508 2(19) &  &  &  & {\multirow{2}{*}{\tablenum{-0.617 945 60}}}& 0.109 86(2) & -0.508 08(2) \\
  &  & GF & -0.508 11(2) & -0.440 235 3(3) &	-0.067 867 7(5) &	-0.508 103 0(7) & & 0.109 843 28(1) & -0.508 102 32(1) \\
  & F & DKB & 55.556 9(8) &  &  &  & {\multirow{2}{*}{\tablenum{24.685 497}}}& 30.871 6(1) & 55.557 0(1) \\ 
  &  & GF & 55.557 2(1) & 25.359 90(2) &  30.197 273(2) & 55.557 17(2) & & 30.871 682(2) & 55.557 179(2) \\ 
\hline
 26 & C & DKB & -0.458 72(9) &  &  &  & {\multirow{2}{*}{\tablenum{-0.497 070 7}}}& 0.038 25(5) & -0.458 82(5) \\
  &  & GF & -0.458 79(1)  & -0.377 228 12(3) & 	-0.081 559 7(5) &	-0.458 787 8(5) & & 0.038 282 9(4) & -0.458 787 8(4) \\
  & F & DKB & 25.371 3(3) &  &  &  & {\multirow{2}{*}{\tablenum{10.809 479 4}}}& 14.561 5(1) & 25.370 9(1) \\ 
  &  & GF & 25.371 03(1) & 11.080 133 05(4) & 14.290 907(2) & 25.371 040(2) & & 14.561 562 1(6) & 25.371 041 5(6) \\ 
\hline
 36 & C & DKB & 0.410 2(1) &  &  &  & {\multirow{2}{*}{\tablenum{-0.388 558 5}}}& -0.021 83(5) & -0.410 38(5) \\
  &  & GF & -0.410 34(1)  & -0.315 349 962 3(19) &	-0.094 992 9(4) &	-0.410 342 8(4) & & -0.021 784 3(3) & -0.410 342 8(3) \\
  & F & DKB & 12.494 8(4) &  &  &  & {\multirow{2}{*}{\tablenum{5.054 839 9}}}& 7.439 7(1) & 12.494 5(1) \\ 
  &  & GF & 12.494 63(2) & 5.168 459 166(5)	& 7.326 183 4(14)	& 12.494 642 6(14) & & 7.439 803 3(4) & 12.494 643 3(4) \\ 
\hline
 54 & C & DKB & -0.348 74(3) &  &  &  & {\multirow{2}{*}{\tablenum{-0.258 689 31}}}& -0.090 09(2) & -0.348 78(2) \\
  &  & GF & -0.348 758(1)  & -0.235 050 084 3(11) &	-0.113 707 7(2) &	-0.348 757 8(2) & & 0.090 068 45(5) & -0.348 757 76(4) \\
  & F & DKB & 5.092 1(3) &  &  &  & {\multirow{2}{*}{\tablenum{1.901 467 1}}}& 3.190 52(4) & 5.091 98(4) \\ 
  &  & GF & 5.092 013(2) & 1.933 405 160(1) &	3.158 609 4(6)	& 5.092 014 6(6) & & 3.190 547 7(2) & 5.092 014 8(2) \\ 
\hline
 82 & C & DKB & -0.294 98(2) &  &  &  & {\multirow{2}{*}{\tablenum{-0.132 956 05}}}& -0.162 04(2) & -0.294 99(2) \\
  &  & GF & -0.294 988 8(2)  & -0.153 987 845 8(9) &	-0.141 000 96(11) &	-0.294 988 81(11) & & -0.162 032 73(5) & -0.294 988 79(5) \\
  & F & DKB & 2.067 76(2) &  &  &  & {\multirow{2}{*}{\tablenum{0.745 897 72}}}& 1.321 87(2) & 2.067 76(2) \\ 
  &  & GF & 2.067 770 03(15) & 0.738 029 089 8(5) & 1.329 740 9(2) &	2.067 770 0(2) & & 1.321 872 39(5) &	2.067 770 12(5) \\ 
\hline
 92 & C & DKB & -0.285 2(1) &  &  &  & {\multirow{2}{*}{\tablenum{-0.096 833 87}}}& -0.188 36(1) & -0.285 19(1) \\
  &  & GF & -0.285 192 0(2)  & -0.132 008 645(1) &	-0.153 183 54(7) &	-0.285 192 19(7) & & -0.188 358 30(2) & -0.285 192 17(2) \\
  & F & DKB & 1.656 26(5) &  &  &  & {\multirow{2}{*}{\tablenum{0.618 726 4}}}& 1.037 51(1) & 1.656 23(1) \\ 
  &  & GF & 1.656 240(2) & 0.598 961 3(1) &	1.057 278(1) &	1.656 239(1) & & 1.037 513 7(1) & 1.656 240 1(1) \\ 
\hline
 100 & C & GF & -0.281 256 9(1) & -0.116 019 00(1) &	-0.165 237 9(1) &	-0.281 256 9(1) & -0.068 173 06 & -0.213 083 87(1)	& -0.281 256 93(1) \\
  & F & GF & 1.437 300 8(2) & 0.534 332 3(2)	 & 0.902 968 5(1)	& 1.437 300 8(3) & 0.565 473 4	& 0.871 827 3(2) & 1.437 300 7(2) \\
\hline
\hline
 
\end{tabular}
}}}
\end{table}
}



% {{\multirow{2}{*}{\tablenum{\tablenum{149.189 230}}}










% \begin{table}[H]
% \caption{
% Many-potential contribution to the self-energy correction for $1S_{1/2}$ (denoted as $a$) state of the hydrogen-like ions, calculated in three ways - directly, using the Sapirstein-Cheng (SC) approach, and using the separation of the two-potential contribution. Results are given in units $F(\alpha Z)$. For $Z=10$ spherical model was used, and for other $Z$'s Fermi model was used, nuclear radii taken from~\cite{se_yerokh}.}
% \fontsize{9pt}{9pt}\selectfont
% \renewcommand{\arraystretch}{1.35}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ ccclllllll } 
% \hline
% \hline
%  & & & \multicolumn{1}{|c|}{direct} & \multicolumn{3}{|c|}{two-pot. scheme} & \multicolumn{3}{|c}{SC scheme} \\ \hline
%  Z & gauge & & $\Delta\varepsilon^{mp}_a$ & $\Delta\varepsilon^{2p}_a$ & $\Delta\varepsilon^{3+}_a$ & $\Delta\varepsilon^{mp}_a$ & $\Delta \tilde{\varepsilon}_{a,p}^{2p}$ & $\Delta \tilde{\varepsilon}_{a}^{3+}$ & $\Delta \varepsilon_a^{mp}$ \\ \hline
%  10 & C & DKB & -0.570 0(8) &  &  &  & {\multirow{2}{*}{\tablenum{-0.791 761 7} & 0.221 95(5) & -0.569 81(5) \\
%   &  & GF & -0.569 8(1)  & -0.519 43(2) & -0.050 350 0(1) & -0.569 78(2) & & 0.221 992 9(1) & -0.569 768 8(1) \\
%   & F & DKB & 188.7(6) &  &  &  & {\multirow{2}{*}{\tablenum{87.239 75} & 101.435 75(2) & 188.675 50(2) \\ 
%   &  & GF & 188.675 3(2) & 89.835 999(2) & 98.839 47(1) & 188.675 47(1) & & 101.435 74(2) & 188.675 49(2) \\ 
% \hline
%  18 & C & DKB & -0.508 2(19) &  &  &  & {\multirow{2}{*}{\tablenum{-0.617 945 60} & 0.109 86(2) & -0.508 08(2) \\
%   &  & GF & -0.508 11(2) & -0.440 235 3(3) &	-0.067 867 7(5) &	-0.508 103 0(7) & & 0.109 843 28(1) & -0.508 102 32(1) \\
%   & F & DKB & 55.556 9(8) &  &  &  & {\multirow{2}{*}{\tablenum{24.685 497} & 30.871 6(1) & 55.557 0(1) \\ 
%   &  & GF & 55.557 2(1) & 25.359 90(2) &  30.197 273(2) & 55.557 17(2) & & 30.871 682(2) & 55.557 179(2) \\ 
% \hline
%  26 & C & DKB & -0.458 72(9) &  &  &  & {\multirow{2}{*}{\tablenum{-0.497 070 7} & 0.038 25(5) & -0.458 82(5) \\
%   &  & GF & -0.458 79(1)  & -0.377 228 12(3) & 	-0.081 559 7(5) &	-0.458 787 8(5) & & 0.038 282 9(4) & -0.458 787 8(4) \\
%   & F & DKB & 25.371 3(3) &  &  &  & {\multirow{2}{*}{\tablenum{10.809 479 4} & 14.561 5(1) & 25.370 9(1) \\ 
%   &  & GF & 25.371 03(1) & 11.080 133 05(4) & 14.290 907(2) & 25.371 040(2) & & 14.561 562 1(6) & 25.371 041 5(6) \\ 
% \hline
%  36 & C & DKB & 0.410 2(1) &  &  &  & {\multirow{2}{*}{\tablenum{-0.388 558 5} & -0.021 83(5) & -0.410 38(5) \\
%   &  & GF & -0.410 34(1)  & -0.315 349 962 3(19) &	-0.094 992 9(4) &	-0.410 342 8(4) & & -0.021 784 3(3) & -0.410 342 8(3) \\
%   & F & DKB & 12.494 8(4) &  &  &  & {\multirow{2}{*}{\tablenum{5.054 839 9} & 7.439 7(1) & 12.494 5(1) \\ 
%   &  & GF & 12.494 63(2) & 5.168 459 166(5)	& 7.326 183 4(14)	& 12.494 642 6(14) & & 7.439 803 3(4) & 12.494 643 3(4) \\ 
% \hline
%  54 & C & DKB & -0.348 74(3) &  &  &  & {\multirow{2}{*}{\tablenum{-0.258 689 31} & -0.090 09(2) & -0.348 78(2) \\
%   &  & GF & -0.348 758(1)  & -0.235 050 084 3(11) &	-0.113 707 7(2) &	-0.348 757 8(2) & & -0.090 068 45(5) & -0.348 757 76(4) \\
%   & F & DKB & 5.092 1(3) &  &  &  & {\multirow{2}{*}{\tablenum{1.901 467 1} & 3.190 52(4) & 5.091 98(4) \\ 
%   &  & GF & 5.092 013(2) & 1.933 405 160(1) &	3.158 609 4(6)	& 5.092 014 6(6) & & 3.190 547 7(2) & 5.092 014 8(2) \\ 
% \hline
%  82 & C & DKB & -0.294 98(2) &  &  &  & {\multirow{2}{*}{\tablenum{-0.132 956 05} & -0.162 04(2) & -0.294 99(2) \\
%   &  & GF & -0.294 988 8(2)  & -0.153 987 845 8(9) &	-0.141 000 96(11) &	-0.294 988 81(11) & & -0.162 032 73(5) & -0.294 988 79(5) \\
%   & F & DKB & 2.067 76(2) &  &  &  & {\multirow{2}{*}{\tablenum{0.745 897 72} & 1.321 87(2) & 2.067 76(2) \\ 
%   &  & GF & 2.067 770 03(15) & 0.738 029 089 8(5) & 1.329 740 9(2) &	2.067 770 0(2) & & 1.321 872 39(5) &	2.067 770 12(5) \\ 
% \hline
%  92 & C & DKB & -0.285 2(1) &  &  &  & {\multirow{2}{*}{\tablenum{-0.096 833 87} & -0.188 36(1) & -0.285 19(1) \\
%   &  & GF & -0.285 192 0(2)  & -0.132 008 645(1) &	-0.153 183 54(7) &	-0.285 192 19(7) & & -0.188 358 30(2) & -0.285 192 17(2) \\
%   & F & DKB & 1.656 26(5) &  &  &  & {\multirow{2}{*}{\tablenum{0.618 726 4} & 1.037 51(1) & 1.656 23(1) \\ 
%   &  & GF & 1.656 240(2) & 0.598 961 3(1) &	1.057 278(1) &	1.656 239(1) & & 1.037 513 7(1) & 1.656 240 1(1) \\ 
% \hline
%  100 & C & GF & -0.281 256 9(1) & -0.116 019 00(1) &	-0.165 237 9(1) &	-0.281 256 9(1) & -0.068 173 06 & -0.213 083 87(1)	& -0.281 256 93(1) \\
%   & F & GF & 1.437 300 8(2) & 0.534 332 3(2)	 & 0.902 968 5(1)	& 1.437 300 8(3) & 0.565 473 4	& 0.871 827 3(2) & 1.437 300 7(2) \\
% \hline
% \hline
% \end{tabular}%
% }
% \centering
% \label{tab:we_yerokh_2p}
% \end{table}

==> we_yerokh_general.tex <==
{\setlength\LTcapwidth{\textwidth}
\renewcommand{\arraystretch}{1.3}
\begin{table}[h]
    \centering
    \caption{\label{tab:we_yerokh}
Individual contributions to the self-energy correction for the $1S_{1/2}$ state of hydrogen-like ions in the Feynman (F)
and Coulomb (C) gauges in $F(\alpha Z)$ units. For $Z=10$ spherical model was used, and for other $Z$'s Fermi model was used, nuclear radii taken from~\cite{se_yerokh}.
         }
{
    \begin{tabular}{
                l@{\quad}
                l@{\quad}
                l@{\quad}
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                S[table-format=3.9(2),group-separator={\;},group-minimum-digits=3]
                 }
\hline
\hline 

\multicolumn{1}{l}{$Z$} & 
\multicolumn{1}{l}{gauge} & &
\multicolumn{1}{c}{$\Delta \varepsilon_a^{0\text{p}}$} &
\multicolumn{1}{c}{$\Delta \varepsilon_a^{1\text{p}}$} & 
\multicolumn{1}{c}{$\Delta \varepsilon_a^{\text{Mp}}$} &
\multicolumn{1}{c}{$\Delta \varepsilon_a$} \\
\hline 
 10 & C & DKB     & {\multirow{2}{*}{\tablenum{5.502 181 5}}} & {\multirow{2}{*}{\tablenum{-0.278 283 7}}} & -0.569 81(5) & 4.654 08(5) \\ 
 &  & GF         & & & -0.569 768 8(1) & 4.654 129 0(1) \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-828.249 50}}} & {\multirow{2}{*}{\tablenum{644.228 14}}} & 188.675 50(2) & 4.654 14(2) \\ 
 &  & GF         & & & 188.675 47(1) & 4.654 11(1) \\ 
 &  & \cite{se_yerokh} &  &  &  & 4.654 129 \\ \hline
 18 & C & DKB     & {\multirow{2}{*}{\tablenum{3.797 152 55}}} & {\multirow{2}{*}{\tablenum{0.155 009 41}}} & -0.508 08(2) & 3.444 08(2) \\ 
 &  & GF         & & & -0.508 102 32(1) & 3.444 059 64(1) \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-192.239 149}}} & {\multirow{2}{*}{\tablenum{140.126 028}}} & 55.557 0(1) & 3.443 9(1) \\ 
 &  & GF         & & & 55.557 179(2) & 3.444 058(2) \\ 
 &  & \cite{se_yerokh} &  &  &  & 3.444 059(1) \\ \hline
 26 & C & DKB     & {\multirow{2}{*}{\tablenum{2.891 040 2}}} & {\multirow{2}{*}{\tablenum{0.351 512 5}}} & -0.458 82(5) & 2.783 73(5) \\ 
 &  & GF         & & & -0.458 787 8(4) & 2.783 764 9(4) \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-74.244 868 3}}} & {\multirow{2}{*}{\tablenum{51.657 591 3}}} & 25.370 9(1) & 2.783 6(1) \\ 
 &  & GF         & & & 25.371 041 5(6) & 2.783 764 5(6) \\ 
 &  & \cite{se_yerokh} &  &  &  & 2.783 765 \\ \hline
 36 & C & DKB     & {\multirow{2}{*}{\tablenum{2.208 571 6}}} & {\multirow{2}{*}{\tablenum{0.481 092 9}}} & -0.410 38(5) & 2.279 28(5) \\ 
 &  & GF         & & & -0.410 342 8(3) & 2.279 321 7(3) \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-31.021 248 6}}} & {\multirow{2}{*}{\tablenum{20.805 926 9}}} & 12.494 5(1) & 2.279 2(1) \\ 
 &  & GF         & & & 12.494 643 3(4) & 2.279 321 6(4) \\ 
 &  & \cite{se_yerokh} &  &  &  & 2.279 322 \\ \hline
 54 & C & DKB     & {\multirow{2}{*}{\tablenum{1.523 080 46}}} & {\multirow{2}{*}{\tablenum{0.607 564 15}}} & -0.348 78(2) & 1.781 86(2) \\ 
 &  & GF         & & & -0.348 757 76(4) & 1.781 886 85(4) \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-9.961 275 6}}} & {\multirow{2}{*}{\tablenum{6.651 147 5}}} & 5.091 98(4) & 1.781 85(4) \\ 
 &  & GF         & & & 5.092 014 8(2) & 1.781 886 7(2) \\ 
 &  & \cite{se_yerokh} &  &  &  & {1.781 887(2)(2)} \\ \hline
 82 & C & DKB     & {\multirow{2}{*}{\tablenum{0.994 837 25}}} & {\multirow{2}{*}{\tablenum{0.787 437 13}}} & -0.294 98(2) & 1.487 29(2) \\ 
 &  & GF         & & & -0.294 988 79(5) & 1.487 285 59(5)  \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-2.952 357 937}}} & {\multirow{2}{*}{\tablenum{2.371 873 437}}} & 2.067 76(2) & 1.487 27(2) \\ 
 &  & GF         & & & 2.067 770 12(5) & 1.487 285 62(5) \\ 
 &  & \cite{se_yerokh} &  &  &  & {\; 1.487 286(16)(3)} \\ \hline
 92 & C & DKB     & {\multirow{2}{*}{\tablenum{0.871 179 70}}} & {\multirow{2}{*}{\tablenum{0.886 500 90}}} & -0.285 19(1) & 1.472 49(1) \\ 
 &  & GF         & & & -0.285 192 17(2) & 1.472 488 43(2) \\ 
 & F & DKB       & {\multirow{2}{*}{\tablenum{-2.141 311 3}}} & {\multirow{2}{*}{\tablenum{1.957 559 5}}} & 1.656 23(1) & 1.472 48(1) \\ 
 &  & GF         & & & 1.656 240 1(1) & 1.472 488 3(1) \\ 
 &  & \cite{se_yerokh} &  &  &  & {1.472 50(1)(2)} \\ \hline
 100 & C & GF     & 0.780 926 90 & 0.996 469 02 & -0.281 256 93(1) & 1.496 138 99(1) \\ 
 & F & GF         & -1.737 050 7 & 1.795 888 8 & 1.437 300 7(2) & 1.496 138 8(1) \\ 
 &  & \cite{se_yerokh} &  &  &  & {1.496 14(7)(47)} \\ \hline
\hline
\end{tabular}
}
\end{table}
}

